Interpretable-by-Design Text Understanding with Iteratively Generated Concept Bottleneck

Black-box deep neural networks excel in text classification, yet their application in high-stakes domains is hindered by their lack of interpretability. To address this, we propose Text Bottleneck Models (TBM), an intrinsically interpretable text classification framework that offers both global and local explanations. Rather than directly predicting the output label, TBM predicts categorical values for a sparse set of salient concepts and uses a linear layer over those concept values to produce the final prediction. These concepts can be automatically discovered and measured by a Large Language Model (LLM) without the need for human curation. Experiments on 12 diverse text understanding datasets demonstrate that TBM can rival the performance of black-box baselines such as few-shot GPT-4 and finetuned DeBERTa while falling short against finetuned GPT-3.5. Comprehensive human evaluation validates that TBM can generate high-quality concepts relevant to the task, and the concept measurement aligns well with human judgments, suggesting that the predictions made by TBMs are interpretable. Overall, our findings suggest that TBM is a promising new framework that enhances interpretability with minimal performance tradeoffs.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/analysis_results.tex <==
\begin{table*}[!t]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|cc|cc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c|}{\textbf{Sentiment}} & \multicolumn{2}{c}{\textbf{Miscellaneous}}  \\\cmidrule{2-5}
\multicolumn{1}{c|}{} & \textbf{CEBaB} & \textbf{Rotten} & \textbf{SNLI} & \textbf{AG News} \\
\midrule
\textbf{Metric} & MSE$\downarrow$ & Acc$\uparrow$ & Acc$\uparrow$ & Acc$\uparrow$ \\\midrule
\textbf{Model (Interpretable)} &&&& \\
DeBERTa-base (\xmark) & \underline{0.250} & 0.863 & 0.795 & \textbf{0.906} \\
GPT-3.5-finetune (\xmark) & \textbf{0.237} & 0.911 & 0.869 & 0.873 \\
GPT-3.5-5shot (\xmark) & 0.362 & \textbf{0.924} & 0.514 & 0.834 \\
GPT-4-5shot (\xmark) & 0.279 & 0.913 & \textbf{0.873} & \underline{0.893} \\\midrule
Concept (Ours) (\checkmark) & 0.359 & 0.891 & 0.617 & 0.715 \\
Concept Ablation (\checkmark) & 0.521 & 0.891 & 0.568 & 0.451 \\
Concept GPT-4 Measurement (\checkmark) & 0.302 & \underline{0.921} & \underline{0.872} & 0.869 \\
\bottomrule
\end{tabular}
}
\caption{Model performance on 4 datasets across two domains: Sentiment and Miscellaneous. \xmark~and \checkmark~denote whether the model is interpretable or not. For each dataset, the highest performance is \textbf{bold}, and the second highest is \underline{underlined}.}
\label{table:model_performance_focused}
\vspace{-0.4cm}
\end{table*}

==> tables/concept_quality_averages.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{l|ccc}
\toprule
\textbf{Metric} & \textbf{Sentiment} & \textbf{NLI} & \textbf{Topic/Misc} \\ \midrule
Redundancy & 3.883 & 3.196 & 3.387 \\
Causal Relationship & 4.737 & 4.214 & 4.402 \\
Leakage & 4.116 & 3.395 & 3.531 \\
Objectivity & 4.405 & 3.981 & 4.217 \\ \bottomrule
\end{tabular}
\caption{Expert concept annotations for concept generation quality on four aspects on a (1-5) Likert scale: 
\textbf{Redundancy} is concept duplication, lower scores indicate repetition; 
\textbf{Causal Relationship} is pertinence to the task, lower scores are associated with spurious concepts; 
\textbf{Leakage} checks if the concept directly performs the task, lower scores indicates leakage; 
\textbf{Objectivity (Obj)} is measurability clarity, with lower scores indicating more subjectivity
}
\label{fig:expert_concept_annotations}
\label{table:domain_averages}
\end{table*}

==> tables/concept_quality_others.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccc|c|ccc|c}
\toprule
\multirow{2}{*}{\textbf{Metric}} & \multicolumn{4}{c|}{\textbf{NLI}} & \multicolumn{4}{c}{\textbf{Topic/Misc}} \\ \cline{2-9} 
 & \textbf{SNLI} & \textbf{MNLI} & \textbf{QNLI} & \textbf{Average} & \textbf{Phishing} & \textbf{SciCite} & \textbf{AG News} & \textbf{Average} \\ \midrule
Redundancy & 2.744 & 3.083 & 1.870 & 3.196 & 3.857 & 4.944 & 3.369 & 3.387 \\
Causal Relationship & 3.425 & 4.250 & 3.259 & 4.214 & 5.000 & 4.889 & 4.797 & 4.402 \\
Leakage & 3.536 & 3.617 & 2.019 & 3.395 & 4.976 & 3.778 & 3.403 & 3.531 \\
Objectivity & 3.678 & 4.300 & 3.019 & 3.981 & 4.357 & 4.833 & 4.814 & 4.217 \\ \bottomrule
\end{tabular}%
}
\caption{Scores for different metrics across various datasets in the NLI and Topic/Misc domains.}
\label{table:other_concept_quality}
\end{table*}

==> tables/concept_quality_sentiment.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ccccccc|c}
\toprule
\multirow{2}{*}{\textbf{Metric}} & \multicolumn{8}{c}{\textbf{Sentiment}} \\ \cline{2-9} 
 & \textbf{CEBaB} & \textbf{Yelp} & \textbf{Hate} & \textbf{Rotten} & \textbf{Amaz} & \textbf{SST2} & \textbf{IMDB} & \textbf{Average} \\ \midrule
Redundancy & 3.508 & 3.982 & 3.524 & 3.771 & 4.800 & 3.389 & 4.208 & 3.883 \\
Causal Relationship & 4.747 & 4.825 & 4.651 & 4.625 & 4.700 & 4.694 & 4.917 & 4.737 \\
Leakage & 4.539 & 4.123 & 4.667 & 4.167 & 4.233 & 3.167 & 3.917 & 4.116 \\
Objectivity & 4.614 & 4.596 & 4.413 & 4.292 & 4.433 & 4.194 & 4.292 & 4.405 \\ \bottomrule
\end{tabular}%
}
\caption{Scores for different metrics across various datasets in the Sentiment domain.}
\label{table:sentiment_concept_quality}
\end{table*}

==> tables/main_results_figure.tex <==
%Average for new on accuracy: 84.8

%Average for new MSE: 0.593

\begin{figure}[!t]
\centering
  \begin{subfigure}{0.47\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{images/Sentiment_Classification.pdf}
  \end{subfigure}
  \begin{subfigure}{0.47\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{images/regression.pdf}
\end{subfigure}
\begin{subfigure}{0.47\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{images/Topic_Classification.pdf}
  \end{subfigure}
  \caption{Average performance on 4 General-domain classification datasets (left), 3 General-domain regression datasets (middle) and 5 Specific-domain classification datasets (right).}
  \label{fig: average performance}
  \vspace{-0.4cm}
\end{figure}



==> tables/main_results_table.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccc|ccc|ccccc}
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{4}{c|}{\textbf{General domain (classification)}} & \multicolumn{3}{c|}{\textbf{General domain (regression)}} & \multicolumn{5}{c}{\textbf{Specific domain (classification)}}  \\\cline{2-13}
\multicolumn{1}{c|}{} & \textbf{Rotten} & \textbf{Amazon} & \textbf{Poem}   & \textbf{SNLI}   & \textbf{Hate}   & \textbf{CEBaB}  & \textbf{Yelp}   & \textbf{AG}     & \textbf{Fake}   & \textbf{SciCite}& \textbf{Partisan}       & \textbf{Patent} \\\hline
\multicolumn{1}{c|}{\textbf{Train Size}}       & 250    & 250    & 250    & 250    & 500    & 250    & 250    & 250    & 250    & 250    & 250    & 500    \\
\multicolumn{1}{c|}{\textbf{Metric}}   & Acc$\uparrow$    & Acc$\uparrow$    & Acc$\uparrow$    & Acc$\uparrow$    & MSE$\downarrow$    & MSE$\downarrow$    & MSE$\downarrow$    & Acc$\uparrow$    & Acc$\uparrow$    & Acc$\uparrow$    & Acc$\uparrow$   & Acc$\uparrow$    \\ \hline
\textbf{Model (Interptable)}  &&&&&&&&&&&&\\
BERT-base (\xmark)   & 0.788  & 0.872  & 0.712  & 0.480  & 1.868  & 0.567  & 0.935  & 0.904  & 0.705  & 0.692  & 0.784  & 0.462  \\
DeBERTa-base (\xmark) & 0.824  & 0.924  & 0.728  & 0.512  & 1.712  & 0.346  & 0.539  & \textbf{0.912} & \underline{0.846}    & \underline{0.776}    & 0.776  & \underline{0.488}    \\
GPT-3.5-finetune (\xmark) & \underline{0.916}    & 0.964  & \textbf{0.820} & \underline{0.864}    & \textbf{1.079} & \underline{0.300}    & \textbf{0.400} & 0.904  & \textbf{0.950} & \textbf{0.764} & \textbf{0.852} & \textbf{0.604} \\
GPT-4-10shot (\xmark)& 0.912  & \textbf{0.980} & 0.628  & \textbf{0.868} & 1.666  & \textbf{0.272} & \underline{0.412}    & \underline{0.908}    & 0.842  & 0.688  & \underline{0.808}    & 0.474  \\\hline
Naive Bayes  (\checkmark)& 0.640  & 0.684  & 0.604  & 0.368  & 2.789  & 1.173  & 1.380  & 0.716  & 0.419  & 0.512  & 0.668  & 0.282  \\
TBM (Ours) (\checkmark)  & \textbf{0.924} & \underline{0.976}    & \underline{0.796}    & \underline{0.864}    & \underline{1.246}    & 0.431  & 0.461  & 0.832  & 0.776  & 0.740  & 0.772  & 0.450 \\
\end{tabular}
}
\caption{Model performance on 12 datasets. \xmark~and \checkmark denote whether the model is interpretable or not. For each dataset, the highest performance is \textbf{bold}, and the second highest is \underline{underlined}.}
\label{table:model_performance}
\vspace{-0.4cm}
\end{table*}

==> tables/measurement_scores.tex <==
\begin{table}[!h]
\centering
\begin{tabular}{l|cc}
\toprule
\textbf{Dataset} & \textbf{Accuracy} & \textbf{Correlation} \\ \midrule
Rotten Tomatoes & 0.4530 & 0.4404 \\
AG News & 0.5425 & 0.2172 \\
CEBaB & 0.5599 & 0.5174 \\ \bottomrule
\end{tabular}
\caption{Accuracy and correlation scores for different datasets.}
\label{table:dataset_measurement_scores}
\end{table}

==> templates/8-Ethical_Considerations.tex <==
\section{Ethics Statement}
\textbf{Potential risks} 
We note that despite being designed to be more interpretable, the system we present in this paper still relies fundamentally on LLMs whose outputs may be unpredictable or unsafe. Accordingly, a proper deployment of our system would require safeguards to reduce the risk of harm if present.

%Intended use: Not all domains may be useful
